BERTnesia: Investigating the capture and forgetting of knowledge in BERT

Probing complex language models has recently revealed several insights into linguistic and semantic patterns found in the learned representations. In this article, we probe BERT specifically to understand and measure the relational knowledge it captures in its parametric memory. While probing for linguistic understanding is commonly applied to all layers of BERT as well as fine-tuned models, this has not been done for factual knowledge. We utilize existing knowledge base completion tasks (LAMA) to probe every layer of pre-trained as well as fine-tuned BERT models(ranking, question answering, NER). Our findings show that knowledge is not just contained in BERT's final layers. Intermediate layers contribute a significant amount (17-60%) to the total knowledge found. Probing intermediate layers also reveals how different types of knowledge emerge at varying rates. When BERT is fine-tuned, relational knowledge is forgotten. The extent of forgetting is impacted by the fine-tuning objective and the training data. We found that ranking models forget the least and retain more knowledge in their final layer compared to masked language modeling and question-answering. However, masked language modeling performed the best at acquiring new knowledge from the training data. When it comes to learning facts, we found that capacity and fact density are key factors. We hope this initial work will spur further research into understanding the parametric memory of language models and the effect of training objectives on factual knowledge. The code to repeat the experiments is publicly available on GitHub.

==> intro.tex <==
\section{Introduction}

Large pre-trained language models like \bert{}~\cite{devlin2018bert} have heralded an \textit{ImageNet} moment for NLP\footnote{https://thegradient.pub/nlp-imagenet/} with not only significant improvements made to traditional tasks such as question answering and machine translation but also in the new areas such as knowledge base completion.
\bert{} has over 100 million parameters and essentially trades-off transparency and interpretability for performance.

\todo{Needs revision}

Probing is a commonly used technique to better understand the inner workings of \bert{} and other complex language models~\cite{dasgupta2018evaluating,ettinger-etal-2018-assessing, tenney2019you}. In general, probing is a procedure that tests if a specific pattern can be decoded from a model's latent embeddings. Therefore, inputs are constructed whose expected output would not be possible to predict without knowledge of that specific pattern.
While language models have been shown to encode a lot of linguistic information -- like local syntax, long-range semantics or even compositional reasoning -- they also acquired factual and relational knowledge from their training process.

\begin{figure}
    \centering
    \includegraphics[width=0.90\textwidth]{updated_plots/money_figure.png}
    \caption{Overview of \bert{} with our proposed layer-wise probing procedure. Given a masked word, the masked language modeling head (i.e., the decoder) will use the \bert{} embeddings to produce a probability distribution over the vocabulary. The figure shows the top 3 tokens for a selection of layers with the correct answer in boldface. We find not all knowledge to be accessible in the last layers -- a significant amount of facts as well as some relationships are better captured at intermediary layers.}
    \label{fig:money_fig_probing_procedure}
\end{figure}

Recently, \citet{petroni2019language} probed \bert{} and other language models for relational knowledge (e.g., \textit{Trump} \textsf{is the president of} the \textit{USA}) in order to determine the potential of using language models as automatic knowledge bases. 
Their approach converted queries in the knowledge base (KB) completion task of predicting arguments or relations from a KB triple into a natural language cloze task, for example, \texttt{[MASK]} \textsf{is the president of} the \textit{USA}.
This is done to make the query compatible with the pre-training masked language modeling (MLM) objective. By considering multiple probe sets (the LAMA probes), they consequently showed that a reasonable amount of knowledge is captured in \bert{}. 

Since language models store factual knowledge in their parametric memory, they can be used in question answering to directly retrieve answers without using additional context \citep{roberts-etal-2020-much, Lewis2021PAQ6M}. This setting is called closed-book question-answering (CBQA). To build more knowledgeable models, it is important to understand how language models acquire, store, and forget factual knowledge. One approach to infuse more factual knowledge into the parametric memory is by enriching the pre-training data with additional knowledge retrieved from a large textual corpus \citep{Guu2020REALMRL}.To the best of our knowledge, the effect and efficiency of training tasks other than language modeling on factual knowledge is largely unexplored.   
Yet, language models are typically fine-tuned to a down-stream task. 
Hence, there are some natural questions that arise from these promising investigations:
\textit{Is there more knowledge in \bert{} than what is reported? What happens to relational knowledge when \bert{} is fine-tuned for other tasks? Is knowledge gained and lost through the layers?\todo{last question does not come naturally}}

\subsection{Our Contribution.} To improve our understanding of the parametric memory, we study the emergence of knowledge through the layers in \bert{} by devising a procedure to estimate knowledge contained in every layer and not just the last (as done by~\citet{petroni2019language}).
While this type of layer-by-layer probing has been conducted for syntactic, grammatical, and semantic patterns; knowledge probing has only been conducted on final layer representations. 
Observing only the final layer (as we will show in our experiments)  (i)  underestimates the amount of knowledge and (ii) does not reveal how knowledge emerges. Our probing procedure is detailed in Figure~\ref{fig:money_fig_probing_procedure}.
Furthermore, we explore how knowledge is impacted when fine-tuning on knowledge-intensive tasks such as question answering and ranking. 
We list the key research questions we investigated and key findings corresponding to them:

\mpara{Research question I: Do intermediary layers capture knowledge not present in the last layer?} (Section~\ref{sec:intermediate}) 
\\ \\
We find that a substantial amount of knowledge is stored in the intermediate layers ($\sim$24\% on average). \\

\mpara{Research question II: Does all knowledge emerge at the same rate? Do certain types of relational knowledge emerge more rapidly?} (Section~\ref{sec:evolution})
% \paragraph{}
\\ \\
We find that not all relational knowledge is captured gradually through the layers with 15\% of relationship types essentially doubling in the last layer and 7\% of relationship types being maximally captured in an intermediate layer. This is further evidence that now all knowledge is accessible in the last layer. \\


\mpara{Research question III: What is the impact of fine-tuning data on knowledge capture?} (Section~\ref{sec:data_size})
% \paragraph{}
\\ \\  
% We find that the dataset size does not play a major role when the training objective is fixed as MLM. Fine-tuning on a larger dataset does not lead to less forgetting.\\
As the capacity to store factual knowledge is limited, training on larger amounts of new data will result in more previous knowledge being forgotten. We also observe the density of factual information in the training data to be a factor when it comes to retaining knowledge.

\mpara{Research question IV: What is the impact of the fine-tuning objective on knowledge capture ? } (Section~\ref{sec:finetuning})
% \paragraph{}
\\ \\
Fine-tuning always causes forgetting. When the size of the dataset is fixed and training objective varies, the ranking model (\rankmarco{} in our experiments) forgets less than the QA model (35\% vs. 53\%). When it comes to acquiring new knowledge from fine-tuning, we find MLM to be more effective than QA and ranking (26.5\% vs. 17.25\% and 16.5\%). \\


==> intro_avi_old.tex <==
\section{Introduction}

Large pre-trained language models like \bert{}~\cite{devlin2018bert} have heralded an \textit{ImageNet} moment for NLP\footnote{https://thegradient.pub/nlp-imagenet/} with not only significant improvements made to traditional tasks such as question answering and machine translation but also in the new areas such as knowledge base completion.
The \bert{} family of language models essentially showcase the need for over-parameterization and modelling long-term interaction in textual input for improved language understanding.
However, improved performance for such models comes at the expense of reduced interpretability.

Language models have been shown to understand linguistic information like local syntax, long-range semantics or even compositional reasoning.
A recent approach called \emph{probing} is one approach to inspect the inner workings of \bert{} and other complex language models for better interpretability~\cite{dasgupta2018evaluating,ettinger-etal-2018-assessing, tenney2019you}. 
In general, probing is a procedure that tests if a specific linguistic information can be decoded from a model's latent embeddings.
Corresponding to the desired linguistic information under examination, probing inputs are constructed to explicitly test the presence of linguistic patterns.


\begin{figure}
    \centering
    \includegraphics[width=0.90\textwidth]{updated_plots/money_figure.pdf}
    \caption{Overview of \bert{} with our proposed layer-wise probing procedure. Given a masked word, the masked language modeling head (i.e., the decoder) will use the \bert{} embeddings to produce a probability distribution over the vocabulary. The figure shows the top 3 tokens for a selection of layers with the correct answer in boldface. We find not all knowledge to be accessible in the last layers -- a significant amount of facts as well as some relationships are better captured at intermediary layers.}
    \label{fig:money_fig_probing_procedure}
\end{figure}

More interestingly, recent studies have confirmed that \bert{} also acquires factual and relational knowledge from their training process.
Seminal work by~\citet{petroni2019language} probed \bert{} and other language models for relational knowledge (e.g., \textit{Trump} \textsf{is the president of} the \textit{USA}) in order to determine the potential of using language models as automatic knowledge bases. 
Their approach converted queries in the knowledge base (KB) completion task of predicting arguments or relations from a KB triple into a natural language cloze task, for example, \texttt{[MASK]} \textsf{is the president of} the \textit{USA}.
This is done to make the query compatible with the pre-training masked language modeling (MLM) objective. 
By considering multiple probe sets (also called as the LAMA probes), they consequently showed that a reasonable amount of knowledge is captured in \bert{}. 
As a consequence, factual knowledge stored in the parametric memory of \bert{} models can be used for knowledge-intensive tasks like question answering and fact checking without the need of additional context~\citep{roberts-etal-2020-much, Lewis2021PAQ6M}.

However, many questions about the information content in the parametric memory of \bert{} are unanswered. 
Firstly, the existing probing methodology focuses on the final layer of \bert{} and could underestimate the knowledge contained in the lower layers. This prompts the question -- \textit{Is there more knowledge in \bert{} than what is reported? }
Secondly, the effect of fine-tuning on the relational knowledge is not clearly understood. In other words -- \emph{What happens to relational knowledge when \bert{} is fine-tuned for other tasks?}
Finally, we study the knowledge evolution through the layers of the parametric memory of \bert{}, that is, we attempt to understand \emph{how knowledge is gained and/or forgotten through the layers of \bert{}?}
To the best of our knowledge, the effect and efficiency of training tasks other than language modeling on factual knowledge is largely unexplored.   

\subsection{Our contribution} 
To improve our understanding of the parametric memory, we extensively study the emergence of knowledge through the layers in \bert{} by devising a procedure to estimate knowledge contained in every layer and not just the last (as done by~\citet{petroni2019language}).
Our probing procedure is roughly sketched in Figure~\ref{fig:money_fig_probing_procedure} that shows the use of a light-weight decoder for the representations at each \bert{} layer.

\mpara{Knowledge containment.} We show that existing studies that observing only the final layer underestimate the amount of factual knowledge in \bert{}'s parametric memory.
Specifically, we find that a substantial amount of knowledge ($\sim24\%$) is stored in the intermediate layers (Section~\ref{sec:intermediate}).

\mpara{Knowledge evolution.} Additionally, we also provide insights into how relational knowledge emerges through \bert{}'s layers.
We find that not all relational knowledge is captured gradually through the layers with 15\% of relationship types essentially doubling in the last layer and 7\% of relationship types being maximally captured in an intermediate layer (Section~\ref{sec:evolution}). This is further evidence that not all knowledge is accessible in the last layer. 

\mpara{Fine-tuning and forgetting.}  We find that fine-tuning always causes forgetting (Section~\ref{sec:finetuning}). 
When the size of the dataset is fixed and training objective varies, the ranking model (\rankmarco{} in our experiments) forgets less than the QA model (35\% vs. 53\%). 
When it comes to acquiring new knowledge from fine-tuning, we find MLM to be more effective than QA and ranking (26.5\% vs. 17.25\% and 16.5\%).

\mpara{Impact of Training data.} We find that the dataset size does not play a major role when the training objective is fixed as MLM. Fine-tuning on a larger dataset does not lead to less forgetting (Section~\ref{sec:data_size}).
As the capacity to store factual knowledge is limited, training on larger amounts of new data will result in more previous knowledge being forgotten. We also observe the density of factual information in the training data to be a factor when it comes to retaining knowledge.



\subsection{Insights and implications.}
We believe that understanding how and under what conditions knowledge is acquired, stored, and forgotten in the parametric memory of \bert{} would help develop better knowledge-intensive models.
On one hand, our findings can help infuse more factual knowledge into the parametric memory is by enriching the pre-training data with additional knowledge retrieved from a large textual corpus~\citep{Guu2020REALMRL}.
On the other hand, our findings can also help design novel retrieval strategies for extracting relevant factual knowledge from the \bert{}'s parametric memory.





==> intro_old.tex <==
\section{Introduction}

Large pre-trained language models like \bert{}~\cite{devlin2018bert} have heralded an \textit{Imagenet} moment for NLP\footnote{https://thegradient.pub/nlp-imagenet/} with not only significant improvements made to traditional tasks such as question answering and machine translation but also in the new areas such as knowledge base completion. 
\bert{} has over 100 million parameters and essentially trades off transparency and interpretability for performance. Loosely speaking, probing is a commonly used technique to better understand the inner workings of \bert{} and other complex language models~\cite{dasgupta2018evaluating,ettinger-etal-2018-assessing}. 
Probing, in general, is a procedure by which one tests for a specific pattern -- like local syntax, long-range semantics or even compositional reasoning -- by constructing inputs whose expected output would not be possible to predict without the ability to detect that pattern. 
While a large body of work exists on probing \bert{} for linguistic patterns and semantics, there is limited work on probing these models for the factual and relational knowledge they store.

Recently, \citet{petroni2019language} probed \bert{} and other language models for relational knowledge (e.g., \textit{Trump} \textsf{is the president of} the \textit{USA}) in order to determine the potential of using language models as automatic knowledge bases. 
Their approach converted queries in the knowledge base (KB) completion task of predicting arguments or relations from a KB triple into a natural language cloze task, e.g., \texttt{[MASK]} \textsf{is the president of} the \textit{USA}.
This is done to make the query compatible with the pre-training masked language modeling (MLM) objective. They consequently showed that a reasonable amount of knowledge is captured in \bert{} by considering multiple relation probes. 
However, there are some natural questions that arise from these promising investigations:
\textit{Is there more knowledge in \bert{} than what is reported? What happens to relational knowledge when \bert{} is fine-tuned for other tasks? Is knowledge gained and lost through the layers?}

\subsection{Our Contribution.} In this paper, we study the emergence of knowledge through the layers in \bert{} by devising a procedure to estimate knowledge contained in every layer and not just the last (as done by~\citet{petroni2019language}).
While this type of layer-by-layer probing has been conducted for syntactic, grammatical, and semantic patterns; knowledge probing has only been conducted on final layer representations. 
Observing only the final layer (as we will show in our experiments)  (i)  underestimates the amount of knowledge and (ii) does not reveal how knowledge emerges. 
Furthermore, we explore how knowledge is impacted when fine-tuning on knowledge-intensive tasks such as question answering and ranking. 
We list the key research questions we investigated and key findings corresponding to them:

\subsubsection{Research question I: Do intermediary layers capture knowledge not present in the last layer?} (Section~\ref{sec:intermediate}) 
\\ \\
We find that a substantial amount of knowledge is stored in the intermediate layers ($\approx24\%$ on average). \\

\subsubsection{Research question II: Does all knowledge emerge at the same rate? Do certain types of relational knowledge emerge more rapidly?} (Section~\ref{sec:evolution})
% \paragraph{}
\\ \\
We find that not all relational knowledge is captured gradually through the layers with 15\% of relationship types essentially doubling in the last layer and 7\% of relationship types being maximally captured in an intermediate layer. \\


\subsubsection{Research question III: What is the impact of fine-tuning data on knowledge capture?} (Section~\ref{sec:data_size})
% \paragraph{}
\\ \\  
We find that the dataset size does not play a major role when the training objective is fixed as MLM. Fine-tuning on a larger dataset does not lead to less forgetting.\\

\subsubsection{Research question IV: What is the impact of the fine-tuning objective on knowledge capture ? } (Section~\ref{sec:finetuning})
% \paragraph{}
\\ \\
Fine tuning always causes forgetting. When the size of the dataset is fixed and training objective varies, the ranking model (\rankmarco{} in our experiments) forgets less than the QA model (35\% vs. 53\%). When it comes to acquiring new knowledge from fine-tuning, we find MLM to be more effective than QA and ranking (26.5\% vs. 16.5\% and 17.25\%). \\

